Fair Cake Division Under Monotone Likelihood Ratios

This work develops algorithmic results for the classic cake-cutting problem in which a divisible, heterogeneous resource (modeled as a cake) needs to be partitioned among agents with distinct preferences. We focus on a standard formulation of cake cutting wherein each agent must receive a contiguous piece of the cake. While multiple hardness results exist in this setup for finding fair/efficient cake divisions, we show that, if the value densities of the agents satisfy the monotone likelihood ratio property (MLRP), then strong algorithmic results hold for various notions of fairness and economic efficiency. Addressing cake-cutting instances with MLRP, first we develop an algorithm that finds cake divisions (with connected pieces) that are envy-free, up to an arbitrary precision. The time complexity of our algorithm is polynomial in the number of agents and the bit complexity of an underlying Lipschitz constant. We obtain similar positive results for maximizing social (utilitarian) and egalitarian welfare. In addition, we show that, under MLRP, the problem of maximizing Nash social welfare admits a fully polynomial-time approximation scheme (FPTAS). Many distribution families bear MLRP. In particular, this property holds if all the value densities belong to any one of the following families: Gaussian (with the same variance), linear, binomial, Poisson, and exponential distributions. Furthermore, it is known that linear translations of any log-concave function satisfy MLRP. Therefore, our results also hold when the value densities of the agents are linear translations of the following (log-concave) distributions: Laplace, gamma, beta, Subbotin, chi-square, Dirichlet, and logistic. Hence, through MLRP, the current work obtains novel cake-cutting algorithms for multiple distribution families.

==> piecewise-linear.tex <==
\section{Envy-Free Cake Division Under Piecewise Linear Valuations}
\label{appendix:piecewise-linear}
In this section we extend the MLRP framework to find envy-free cake divisions (with disconnected pieces and up to an arbitrary precision) for piecewise linear value densities.\footnote{A function is said to be piecewise linear iff it can be expressed as a union of a finite number of linear functions. Hence, piecewise linear densities contain a finite number of breakpoints and do not necessarily satisfy MLRP.} The work of Kurokawa et al.~\cite{kurokawa2013cut} shows that if there are $k \geq 1$ breakpoints in total across all $n$ agents' piecewise linear value densities, then an envy-free cake division can be computed using $\mathcal{O}\left(n^6k \ln k\right)$ Robertson-Webb queries. We provide an improved query complexity dependence on $n$. Specifically, we show that (up to an arbitrary precision) an envy-free cake division can be found using $\mathcal{O}\left(n^2 k \log^2 (k U) \right) $ queries (Theorem \ref{theorem:PL-EF}); here $U \geq 1$ is an upper bound on the value densities, i.e., $f_i(x) \leq U$ for all $x \in [0,1]$ and $i \in [n]$.


%Assuming that there are bounded breakpoints across all agents' piecewise linear value densities, we develop a query-efficient algorithm for finding envy-free cake divisions in the Robertson-Webb query model. Previously for this setting,
%Our technique  enables us to improve this bound and develop an algorithm that requires $\mathcal{O}(n^2k \log^2 (kU)) $ queries to find an envy-free cake division (up to an arbitrary precision); here, $U\geq 1$ is an upper bound of the value-densities.

%For a cake-division instance $\Cake$ and a precision parameter $\eta>0$, $\textsc{PL-EF}(0,1)$ finds an $\eta$-envy-free ($\eta$-EF) cake division of $\Cake$. Denote $U \geq 1$ to be an upper bound of value densities, i.e., $f_i(x) \leq U$ for all $x \in [0,1]$ and $i \in [n]$. We develop a recursive algorithm $\textsc{PL-EF}(a,b)$ that begins with dividing the interval $[a,b]$ into two equal halves and running \Bin \ on both halves separately for at most some specific number of iterations. Note that we remove agents from the corresponding halves of $[a,b]$ who value the sub-intervals $[a,(a+b)/2]$ and $[(a+b)/2,b]$ for no more than $\widehat{\eta} := \left(\frac{\eta}{k}\right)^2 \frac{1}{U}$. After the execution of \Bin, \  Algorithm~\ref{alg:PL-EF} performs the following verification for both halves, and failure in which leads to a recursive call on that half: 

% ``Was \Bin  \ successful in inducing an $\widehat{\eta}$-EF cake division of $[a,(a+b)/2]$ and $[(a+b)/2,b]$?"

%Lemma~\ref{lemma:recurse} proves that if Algorithm~\ref{alg:PL-EF} recurses on any of the two halves of an interval $[a,b]$ then that half of $[a,b]$ must contain at least one breakpoint of some value-density function. Moreover, if the algorithm receives positive answer to the verification on any half of $[a,b]$, then the recursion on that half terminates and the corresponding allocation is added to the final cake division. We prove (in Theorem~\ref{theorem:PL-EF}) that the cake division $\mathcal{D} = \{D_1, D_2, \dots, D_n\}$ formed by joining all the allocations returned by these recursive calls of $\textsc{PL-EF}(0,1)$ is $\eta$-EF, and we establish a polynomial bound on the query complexity of finding such a cake division.

Our recursive algorithm $\textsc{PL-EF}(a,b)$ aims to compute envy-free divisions for the left and right half of the given interval $[a,b]$, respectively, and then takes the union of these divisions to obtain a fair one for $[a,b]$. Towards this end, if $\Bin$ (Algorithm \ref{alg:BinSearch}) by itself finds (in a specified number of iterations) a division of $[a,(a+b)/2]$ wherein the envy is appropriately small, then $\textsc{PL-EF}(a,b)$ does not recurse over this subinterval, otherwise it does. Identical steps are executed for the right half $[(a+b)/2,b]$. 

Lemma~\ref{lemma:recurse} below shows a recursive call is made only if the subinterval under consideration contains one or more breakpoints. Indeed, if all the value densities are linear within, say, $[a,(a+b)/2]$, then $\Bin$ will necessarily find the desired division, and $\textsc{PL-EF}(a,b)$ will not recurse on $[a,(a+b)/2]$. Furthermore, note that if the length of the interval (i.e., $|b-a|$) is small enough, then the Lipschitz continuity of the densities implies that any division will have appropriately small envy. Using these observations we can bound the total number of recursive calls of $\textsc{PL-EF}(0,1)$, i.e., establish the stated upper bound on the query complexity of finding an envy-free partition (up to an arbitrary precision) of the cake $[0,1]$ for piecewise linear densities. 

Throughout this section, we will use $k \geq 1$ to denote the total number of breakpoints across the piecewise linear $f_i$s and $U \geq 1$ to denote an upper bound on these densities, i.e., $f_i(x) \leq U$ for all $x \in [0,1]$ and $i \in [n]$. Also, for parameter $\eta >0$, we will say that a division $\mathcal{D}=\{D_1, \ldots, D_n\}$ is $\eta$-envy-free iff $v_i(D_i) \geq v_i (D_j) - \eta$ for all $i, j \in [n]$.

\begin{algorithm}
{\bf Input:} A cake-division instance, $\Cake = \langle [n], \{f_i \}_{i} \rangle$, with piecewise linear densities, in the Robertson-Webb query model. \\ %Write $k$ to denote the total number of breakpoints across $f_i$s and $U \geq 1$ to denote an upper bound on the densities. Also, let $\eta >0$ be the precision parameter. \\ %(i.e., $f_i(x) \leq U$ for all $x \in [0,1]$ and $i \in [n]$) \\
{\bf Output:} An $\eta$-envy-free cake division $\mathcal{D} = \{ D_1,\ldots, D_n\} $
\caption{\textsc{PL-EF}$(a,b)$}
\label{alg:PL-EF}
\begin{algorithmic}[1]
\STATE  Set $\widehat{\eta} \coloneqq \left( \frac{\eta}{k} \right)^2 \frac{1}{U}$ and $\lambda \coloneqq \max\left\{U, \frac{U}{\widehat{\eta}}, \frac{1}{\widehat{\eta}} \right\}$.
\STATE \label{step:small-length} If $|b-a| \leq \frac{\eta^2}{k^2 U^2}$, then return division $\{D_j\}_{j=1}^n$, with $D_1= [a, b]$ and $D_i = \emptyset$ for all $i >1$, and exit. 
\STATE  \label{step:prep} Let $K_L \coloneqq \left\{i \in [n] : \Eval_i\left(a, \frac{a+b}{2}\right) \geq \widehat{\eta} \right\}$. Normalize the valuations of the agents in  $K_L$ over $[a,b]$ and compute a potential MLRP order among these agents using Lemma \ref{MLRPorder}. 
\STATE \label{step:subroutine} With this order in hand and for parameter $\delta \coloneqq \frac{\widehat{\eta}}{\lambda}$, run $\Bin$ (Algorithm \ref{alg:BinSearch}), for at most $2 n \log \left( \frac{2 \lambda}{\widehat{\eta}}\right)$ iterations, over the interval $[a, (a+b)/2]$ and with agents $K_L$. 
\STATE \label{step:ef} If Step \ref{step:subroutine} is unable to find an $\widehat{\eta}$-envy-free allocation, then set $\{L_1, L_2, \ldots, L_n\} \coloneqq \textsc{PL-EF} \left(a, \frac{a+b}{2}\right)$, else set $\{L_1, L_2, \ldots, L_n\}$ as the $\widehat{\eta}$-envy-free computed in the previous step. 
%successfully finds an $\widehat{\eta}$-envy-free allocation $\{L_1, L_2, \ldots, L_n\}$ of the interval $[a, \frac{a+b}{2}]$}, then go to step \ref{step:repeatright}.
\STATE  Repeat Steps \ref{step:prep} to \ref{step:ef} for the right half $[\frac{a+b}{2},b]$ and compute allocation $\mathcal{R} = \{R_1, R_2, \ldots, R_n\}$. 
\RETURN \label{step:righthalf} cake division $\mathcal{D} = \{ L_i \cup R_i\}_{i=1}^n$.
\end{algorithmic}
\end{algorithm}

\begin{lemma} \label{lemma:recurse}
Consider a cake-division instance with piecewise linear value densities and an interval $[a,b] \subseteq [0,1]$. If there are no breakpoints in the left half of the interval $[a, (a+b)/2]$, then Step \ref{step:subroutine} succeeds in finding an $\widehat{\eta}$-envy-free division and, hence, $\textsc{PL-EF}(a,b)$ does not recurse on $[a, (a+b)/2]$. An identical claim holds for the right half $[(a+b)/2, b]$. 
\end{lemma}
\begin{proof}
%a recursive call is made in $\textsc{PL-EF}(a,b)$ only if the subinterval under consideration (i.e., either $[a, (a+b)/2]$ or $[(a+b)/2, b]$) contains one or more breakpoints.
%We will prove the contrapositive form of the lemma, i.e., show that if there are no breakpoints in, say, $[a, (a+b)/2]$ then Step \ref{step:subroutine} succeeds in finding an $\widehat{\eta}$-envy-free division and, hence, $\textsc{PL-EF}(a,b)$ will not recurse on $[a, (a+b)/2]$. 
We note that, in Step \ref{step:subroutine} of $\textsc{PL-EF}(a,b)$, $\Bin$ is executed  over the set of agents $K_L \coloneqq \{i \in [n] : \Eval_i\left(a, \frac{a+b}{2}\right) \geq \widehat{\eta} \}$. Since there are no breakpoints in $[a, (a+b)/2]$, the value density of each agent in this subinterval is linear. Moreover, for each agent in $K_L$ the cut and eval queries are $\lambda$-Lipschitz: \textcolor{red}{this follows from the fact that...}

Therefore, via Lemma \ref{RDcomputation}, we get that in Step \ref{step:subroutine} $\Bin$ finds an $\left( \frac{\widehat{\eta}}{\lambda} \right)$-ripple division $\mathcal{L} = \{L_1,\ldots, L_n\}$ in at most $2 n \log \left( \frac{2 \lambda}{\widehat{\eta}}\right)$ iterations. Linear densities always satisfy MLRP, hence, as in the proof of Theorem \ref{theorem:EFdivision}, we get that $\mathcal{L}$ is an $\widehat{\eta}$-envy-free division. In such a case $\textsc{PL-EF}(a,b)$ will not recurse on $[a, (a+b)/2]$ and the lemma stands proved. 
 \end{proof}
%when executed over the entire cake, i.e., the recursive calls made by $\textsc{PL-EF}(0,1)$.
We next upper bound the number of recursive calls made by the algorithm. For precision parameter $\eta >0$ and density upper bound $U \geq 1$, write $B \coloneqq 2 \log \left( \frac{kU}{\widehat{\eta}} \right)$ and $\widehat{\eta} \coloneqq \left(\frac{\eta}{k}\right)^2 \frac{1}{U}$. 

Also, let $N(k', \ell)$ denote the maximum number of nodes in the recursion tree obtained by executing $\textsc{PL-EF}(\cdot)$ on any interval with  
$k'$ breakpoints (of the piecewise linear densities) and of length $\frac{1}{2^{B + 1 -\ell}}$. Hence, the overall recursion tree obtained under $\textsc{PL-EF}(0,1)$ contains at most $N(k, B+1)$ nodes (calls). The following lemma implies the useful upper bound $N(k, B + 1) \leq k (B+1)$. 

%The following lemma shows that $N(k', \ell) \leq k' \ell$ for all $k' \geq 1$ and $\ell \in \{0, 1, \ldots, B\}$. 
%Towards analyzing Algorithm~\ref{alg:PL-EF}, we provide a bound on the maximum number of recursive calls made by $\textsc{PL-EF}(0,1)$. Consider a cake-division instance with value-density functions having $k \geq 1$ breakpoints over an interval of length $\frac{1}{2^{B+1-\ell}}$ for $\ell \in [\ceil{B+1}]$. Here for a given precision parameter $\eta>0$, let us define $B+1 \coloneqq \log \frac{U}{\widehat{\eta}}$ and $\widehat{\eta} \coloneqq \left(\frac{\eta}{k}\right)^2 \frac{1}{U}$. Write $N(k, \ell)$ to denote the maximum number of recursive calls made by $\textsc{PL-EF}(0,1)$. Lemma~\ref{lemma: recursive-calls} gives an upper bound on the quantity $N(k, \ell)$.


 
 \begin{lemma} \label{lemma: recursive-calls}
 %	Let $\Cake= \langle [n], \{f_i \}_{i \in [n] } \rangle $ be a cake-division instance in which the value-density functions are piecewise linear with $k$ breakpoints over an interval of length $\frac{1}{2^{B+1-\ell}}$. Then for any $k \geq 1$ and $ \ell \in \{0, 1,2, \ldots, \ceil{B+1}\}$, we have $N(k, \ell) \leq k \ell$.
 	% 	 Here for a given precision parameter $\eta>0$, we define $B+1 \coloneqq \log \frac{U}{\widehat{\eta}}$ and $\widehat{\eta} \coloneqq \left(\frac{\eta}{k}\right)^2 \frac{1}{U}$.
For all $k' \geq 1$ and $\ell \in \{1, \ldots, B\}$, we have $N(k', \ell) \leq k' \ell$. 
 \end{lemma}
\begin{proof}
We prove the lemma via induction on $k'$ and $\ell$. In particular, consider an interval $[a,b]$ with $k'$ breakpoints and of length  $\frac{1}{2^{B+1-\ell}}$. 

%Note that if $\ell = B$, i.e., the length of the interval is $\frac{1}{2^B} = \frac{\eta^2}{k^2 U^2}$, then $\textsc{PL-EF}(a, b)$ will certainly not recurse (Step \ref{step:small-length}). 


%To begin with, note that there are exactly two scenarios where $\textsc{PL-EF}(a,b)$ terminates and does not recurse on $[a,b]$: 
%\begin{enumerate} [noitemsep]
%\item[(i)] If there are no breakpoints, i.e., $k'=0$ in $[a,b]$ (by Lemma~\ref{lemma:recurse}). 
%Here, the value-densities are linear over $[a,b]$, and hence satisfy MLRP.  We can therefore apply Theorem~\ref{theorem:EFdivision}  to find $\widehat{\eta}$-EF allocation of $[a,b]$.
%\item  [(ii)] If the interval length of $[a,b]$ is at most $\frac{\eta^2}{k^2 U^2}= \frac{1}{2^{B+1}}$ (see Step~\ref{step:small length} of Algorithm~\ref{alg:PL-EF}). 
		
	%	Here, each agent values the interval $[a,b]$ for at most $\widehat{\eta}$. Note that, $\{\Eval_i\}_i$ are $U$-Lipschitz (Proposition~\ref{Lip}), and hence we have $v_i(a,b) \leq  U (\frac{\eta^2}{k^2 U^2}) = \widehat{\eta}$ for all $i \in [n]$. Therefore, the allocation returned in Step~\ref{step:agent1} (of Algorithm~\ref{alg:PL-EF}) is $\widehat{\eta}$-EF..
	%\end{enumerate}
	
To prove the base case of induction, observe that if $[a,b]$ contains a single breakpoint, i.e., $k'=1$, then $\textsc{PL-EF}(a,b)$ will only recurse either on the left half or the right half of $[a,b]$ that contains the breakpoint (Lemma \ref{lemma:recurse}). Furthermore, this process can continue for at most $\ell$ recursive calls, after which the interval length becomes $\frac{1}{2^{B}} = \frac{\eta^2}{k^2 U^2}$ (see Step \ref{step:small-length}). Therefore, we have $N(1,\ell) \leq \ell$ for all $\ell \in [B]$. %Furthermore, Step~\ref{step:small length} of Algorithm~\ref{alg:PL-EF} implies that $N(k,0) = 0$ for all $k \geq 1$, and hence establishing the base case.
   
We will now assume that the statement holds true for $N(t, \ell-1)$ with $t \leq k'$, and will inductively prove it for $N(k',\ell)$. We break our analysis in the following two cases depending on the distribution of the breakpoints in $[a,b]$: 
\begin{enumerate}[noitemsep]
\item[(i)] Either the left or the right half of $[a,b]$ contains no breakpoint. In such a case, $\textsc{PL-EF}(a,b)$ can recurse only on the half that contains all $k'$ breakpoints, while the other half terminates. Hence, we have $N(k', \ell)  = N(k', \ell-1) +1$.
\item[(ii)] The left half $[a, \frac{a+b}{2}]$  contains $k_1 \geq 1$ breakpoints and right half $[\frac{a+b}{2},b]$ contains $k_2\geq 1$ breakpoints, with $k_1+k_2=k$. In such a setting, we can write $N(k, \ell)  = N(k_1, \ell-1) +N(k_2, \ell-1)+1$.
\end{enumerate}

Therefore, we can bound $N(k, \ell)$ as
\begin{align*}
N(k, \ell) & \leq \max\{ N(k,\ell-1)+1, N(k_1, \ell-1) +N(k_2, \ell-1)+1\} \\
& \leq \max\{  k(\ell-1) +1, k_1(\ell-1) + k_2(\ell-1)+1\} \tag{by induction hypothesis} \\
& \leq \max\{k \ell, k(\ell-1) +1\}\\
& \leq k \ell
\end{align*}
  
   Therefore, if $N(t, \ell-1) \leq t(\ell-1)$ for all $t \leq k$ then we have $N(k, \ell) \leq k \ell.$
   
    Finally, we will assume that the statement holds true for $N(t-1, h)$ with $t\leq k$ and $h \leq \ell$, and will inductively prove it for $N(k,\ell)$. We once again break our analysis in the following two complementary and exhaustive cases:
    \begin{enumerate}
    	\item [(i)] For $\ell$ consecutive recursive calls, either the left or right half of the considered sub-intervals contain no breakpoint. That is, we can write $N(k, \ell) = N(k,0)+\ell$.
    	\item [(ii)] For $m < \ell$ consecutive recursive calls, either the left or right half of the considered sub-intervals contain no breakpoint (i.e., we have  $ N(k, \ell)  = N(k, \ell-m) +m$). And after $m$ recursive calls, there are $k'_1 \geq 1$ breakpoints in the left half and $k'_2 \geq 1$ breakpoints (with $k'_1+k'_2=k$) in the right half of the current sub-interval of length $\frac{1}{2^{B+1-(\ell-m)}}$. We can therefore write $ N(k, \ell) = N(k, \ell-m) +m = N(k'_1,\ell-m-1)+N(k'_2,\ell-m-1)+m+1$.
    \end{enumerate}

  Overall we can bound $N(k, \ell)$ as
    \begin{align*}
 N(k, \ell) & \leq \max\{N(k,0)+\ell, N(k'_1,\ell-m-1)+N(k'_2,\ell-m-1)+m+1\} \\
 & \leq \max\{  \ell , k'_1(\ell-m-1) + k'_2(\ell-m-1)+m+1\} \tag{by induction hypothesis and the base case} \\
 & \leq \max\{ \ell, k (\ell-m-1) + m+1\}\\
 & \leq k \ell
 \end{align*}
	Therefore, if $N(t-1, h) \leq (t-1)h$ for all $t\leq k$ and $h \leq \ell$, we have for $N(k,\ell) \leq k \ell$.
    This completes our induction argument  and establishes the stated claim.
\end{proof}


Using Lemma~\ref{lemma: recursive-calls}, next we upper bound the maximum number of intervals assigned to any agent by $\textsc{PL-EF}(0,1)$.

\begin{lemma} \label{lemma:number of intervals}
Let $\Cake=\langle [n], \{f_i \}_i \rangle$ be a cake-division instance with piecewise linear value densities that have $k$ breakpoints. Then, the cake division $\mathcal{D} = \{D_1, \ldots, D_n\}$ computed for $\Cake$ by $\textsc{PL-EF}(0,1)$ (Algorithm~\ref{alg:PL-EF}) satisfies 
\begin{align*}
|D_i| \leq 2 N(k,B+1) &  \leq  2 k(B+1) \quad \text{ for all } i \in [n].
%|D_1| \leq 2N(k,B+1) &  \leq 2k(B+1).
\end{align*}
\end{lemma}
\begin{proof}
In $\textsc{PL-EF}(\cdot)$, at each node of the recursion tree at most two additional intervals are assigned to any agent. Since the number of nodes in the recursion tree is at most $N(k, B+1)$, the lemma follows.
%At each node of the Note that the quantity $N(k, B+1)$ represents the maximum number of recursive calls made by $\textsc{PL-EF}(0,1)$ for a cake-division instance with piecewise linear value-densities having at most $k$ breakpoints over a cake of length $\frac{1}{2^{B+1-(B+1)}}=1$. The proof of Proposition~\ref{proposition:number of intervals} now follows via induction on $k$ (similar to arguments used in Lemma~\ref{lemma: recursive-calls}), and the observation that one extra interval may be assigned to agent $1$ at each terminating call (Step~\ref{step:agent1} of Algorithm~\ref{alg:PL-EF}). 
\end{proof}

 
 
Theorem~\ref{theorem:PL-EF} presents our main result of this section. % and establishes a bound of $\mathcal{O}(n^2k \log^2 ( kU)) $ on the query complexity of computing an envy-free cake division, up to an arbitrary precision, in the Robertson-Webb query model for instances with piecewise linear value-densities having $k$ breakpoints.

\begin{theorem} \label{theorem:PL-EF}
Let $\Cake = \langle [n], \{f_i \}_{i} \rangle $ be a cake-division instance in which the value densities are piecewise linear and have $k$ breakpoints overall. Then, for precision parameter $\eta>0$ and in the Robertson-Webb query model, an $\eta$-envy-free cake division of $\Cake$ can computed using $\mathcal{O}\left( n^2k \log^2 \left(\frac{kU}{\eta}  \right) \right) $ queries. Here $U \geq 1$ is an upper bound of value densities, i.e., $f_i(x) \leq U$ for all $x \in [0,1]$ and $i \in [n]$.
 \end{theorem}

\begin{proof}
We will first prove that Algorithm~\ref{alg:PL-EF} outputs an $\eta$-envy-free cake division $\mathcal{D} = \{D_1, D_2, \dots, D_n\}$. 
Recall that $\widehat{\eta} \coloneqq \left(\frac{\eta}{k}\right)^2 \frac{1}{U}$, and $B+1 \coloneqq \log \frac{U}{\widehat{\eta}}$. Also, at any terminating call in $\textsc{PL-EF}(\cdot)$, an $\widehat{\eta}$-envy-free division (of some subinterval) is assigned among the agents. Specifically, in Step \ref{step:small-length}, the fact that $|b-a| \leq \frac{\eta^2}{k^2 U^2}$ and the bound $f_i(x) \leq U$ (for all $x \in [0,1]$) imply that $v_i(a, b) \leq \widehat{\eta}$ for all $i \in [n]$ and, hence, the returned division is $\widehat{\eta}$-envy-free.

The allocation $\{D_1, D_2, \dots, D_n\}$ computed by $\textsc{PL-EF}(0,1)$ is the union of $2 k(B+1)$ such $\widehat{\eta}$-envy-free divisions (Lemma \ref{})

Let us define  Recall that, at each terminating call (see Steps~\ref{step:small length} and \ref{step:update}) during the execution of Algorithm~\ref{alg:PL-EF}, an $\widehat{\eta}$-EF allocation is added to the cake division $\mathcal{D}$.  Hence, envy between agents in the cake division $\mathcal{D}$ can be bounded by summing their envy in each of the (at most) $2k(B+1)$ $\widehat{\eta}$-EF allocations that are added to $\mathcal{D}$. For any $i,j \in [n]$, we have
 	%\footnote{If the value densities satisfy MLRP in some sub-interval $[c,d] \subseteq [0,1]$ during a recursive call, then $\lambda = \max\{U, \frac{U}{\eta}, \frac{1}{\eta}\}$ is indeed a Lipschitz constant for the cut and eval queries.}
 	\begin{align*}
    |v_i(D_i) - v_i(D_j)| & \leq 2k(B+1) \widehat{\eta} \tag{by Proposition~\ref{proposition:number of intervals}} \\
    & \leq \frac{2\eta^2}{k} \frac{1}{U} \log\left(\frac{k^2 U^2}{\eta^2}\right) \tag{by definition of $B+1$ and $\widehat{\eta}$} \\
    & \leq \eta \left(\frac{\eta}{k U}\right) 4 \log \left(\frac{k U}{\eta}\right) \\
    & \leq \eta
 	\end{align*}
 	where the last inequality follows from the fact that $4 \log x \leq x$ for all $x \geq 4$; setting $ x=\frac{k U}{\eta} \geq 4$. Therefore, $\mathcal{D}$ is an $\eta$-EF cake division in $\Cake$.
 	
 	Next, we will analyze the query complexity of Algorithm~\ref{alg:PL-EF}. Note that Lemma~\ref{lemma: recursive-calls} proves that the maximum number of recursive calls made by $\textsc{PL-EF}(0,1)$ is $N(k, B+1) =k(B+1)$. Recall that, $\textsc{PL-EF}(a,b)$ performs identical operations on the two equal halves (see Step~\ref{step:righthalf}) of interval $[a,b]$ during its recursive call on $[a,b]$. Hence, we can bound the maximum number of queries required for the left half $[a, (a+b)/2]$ and multiply it by $2$ to get the total number of queries made by $\textsc{PL-EF}(a,b)$.
 	 
 	To begin with, it requires $n$ queries to find the set $K_L$ (in Step~\ref{step:subroutine}) of agents valuing the interval $[a, \frac{a+b}{2}]$ for no more than $\widehat{\eta}$. Next, at most $n$ queries are made to normalize the value-densities of agents over $[a,\frac{a+b}{2}]$, and another $n$ queries to compute a potential candidate for the MLRP order for agents in $[n] \setminus K_L$ (Step~\ref{step:subroutine}). Then, \Bin \ is executed for at most $2(n-1) \log \left(\frac{2 \lambda}{\widehat{\eta}}\right)$ number of iterations (in Step~\ref{step:subroutine}), where each such iteration requires $2n$ queries.
 	Finally, it takes at most $n^2$ queries to verify if an $\widehat{\eta}$-EF allocation is computed (in Step~\ref{step:ef}). Overall, the maximum number of queries, denoted by $Q(n,k)$, made by Algorithm~\ref{alg:PL-EF} can be bounded as,
 	\begin{align*}
 	Q(n,k) & \leq k(B+1) \left( 2 \left( n+n+ 2n \left(2(n-1) \log \left(\frac{2  \lambda}{\widehat{\eta}}\right)\right) + n^2 \right) \right) \\
 	& \leq k(B+1) \left(14n^2\log \left(\frac{2 \lambda}{\widehat{\eta}}\right) \right) \\
 	& \leq \mathcal{O}(n^2 k) \log \left(\frac{ k^2 U^2}{\eta^2}\right)  \log \left(\frac{2 \lambda k^2U}{\eta^2}\right) \\
 	& \leq \mathcal{O}(n^2 k) \log \left(\frac{  kU}{\eta}\right) \left( \log (2\lambda )+2 \log \left(\frac{ kU}{\eta}\right)\right) \tag{since $U \geq 1$} \\
 	& \leq  \mathcal{O}(n^2 k) \left( 2\log^2 \left(\frac{kU}{\eta}\right) + \log (2\lambda )\log \left(\frac{kU}{\eta}\right) \right) 
 	\end{align*}
 	Recall that $\lambda = \max\{U, \frac{k^2 U}{\eta^2},\frac{k^2 U^2}{\eta^2} \}$. Assuming that the precision parameter $\eta \leq 1$, we have $\lambda =  \frac{k^2U^2}{\eta}$, and hence $\log(2 \lambda) = \log \left(\frac{2k^2U^2}{\eta^2} \right)$,
 	since $U \geq 1$. That is, we have $\log(2 \lambda) = \mathcal{O} \left(\log \left(\frac{kU}{\eta}\right)\right)$.
 	Overall, we obtain the required bound, $Q(n,k) = \mathcal{O}\left( n^2k \log^2 \left(\frac{kU}{\eta}  \right) \right)$.
 	
 	
 	Hence, Algorithm~\ref{alg:PL-EF} requires  $\mathcal{O}\left( n^2k \log^2 \left(\frac{kU}{\eta}  \right) \right) $queries  to compute an $\eta$-EF cake division. Theorem~\ref{theorem:PL-EF} now stands proved.
 \end{proof}


The query complexity obtained via Theorem~\ref{theorem:PL-EF} implies that the precision parameter $\eta$ can be driven exponentially close to zero, in queries that is polynomial in $\log \frac{1}{\eta}$ (i.e., in the bit complexity of $\eta$). Hence, we
can find an envy-free cake division, up to arbitrary precision, using $\mathcal{O}(n^2k \log^2 (kU)) $ queries.



